Dimension and Relative Frequencies

We show how to calculate the finite-state dimension (equivalently, the finite-state compressibility) of a saturated sets $X$ consisting of {\em all} infinite sequences $S$ over a finite alphabet $\Sigma_m$ satisfying some given condition $P$ on the asymptotic frequencies with which various symbols from $\Sigma_m$ appear in $S$. When the condition $P$ completely specifies an empirical probability distribution $\pi$ over $\Sigma_m$, i.e., a limiting frequency of occurrence for {\em every} symbol in $\Sigma_m$, it has been known since 1949 that the Hausdorff dimension of $X$ is precisely $\CH(\pi)$, the Shannon entropy of $\pi$, and the finite-state dimension was proven to have this same value in 2001. The saturated sets were studied by Volkmann and Cajar decades ago. It got attention again only with the recent developments in multifractal analysis by Barreira, Saussol, Schmeling, and separately Olsen. However, the powerful methods they used -- ergodic theory and multifractal analysis -- do not yield a value for the finite-state (or even computable) dimension in an obvious manner. We give a pointwise characterization of finite-state dimensions of saturated sets. Simultaneously, we also show that their finite-state dimension and strong dimension coincide with their Hausdorff and packing dimension respectively, though the techniques we use are completely elementary. Our results automatically extend to less restrictive effective settings (e.g., constructive, computable, and polynomial-time dimensions).

==> bigpage.tex <==
\oddsidemargin  0.0in
\evensidemargin 0.0in
\textwidth      6.5in
\headheight     0.0in
\topmargin      -0.2in
\textheight 	8.7in



==> commands.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumerate}

% Decision Problems
%\newcommand{\SAT}{\mathrm{SAT}}
%\newcommand{\MAXSAT}{\mathrm{MAXSAT}}
%\newcommand{\MAXTSAT}{\mathrm{MAX3SAT}}
\newcommand{\MAXSAT}{\textsc{MaxSat}}
\newcommand{\MAXTSAT}{\textsc{Max3Sat}}
\newcommand{\SAT}{{\rm SAT}}
\newcommand{\MAXCLIQUE}{\textsc{MaxClique}}
\newcommand{\CLIQUE}{\textsc{Clique}}

% Proof Commands
\newcommand{\PROOF}{\begin{proof}}%{{\noindent\bf{\em Proof:\/}~~}}
\newcommand{\PROOFSKETCH}{{\noindent\bf{\em Proof sketch:\/}~~}}
\newcommand{\QED}{\end{proof}}
\newcommand{\QEDbox}{\nolinebreak{\hfill $\square$}\vspace*{0.3cm}}

% Miscellaneous
\newcommand{\third}{3^{\mathrm{rd}}}
\newcommand{\second}{2^{\mathrm{nd}}}
\newcommand{\first}{1^{\mathrm{st}}}
\newcommand{\Prob}{\mathrm{Prob}}
\newcommand{\floor}[1]{ \left\lfloor #1 \right\rfloor }
\newcommand{\ceil}[1]{ \left\lceil #1 \right\rceil }
\newcommand{\range}{\mathrm{range}}
\newcommand{\mysets}[2]{ \{ #1 \;|\; #2  \} }
\newcommand{\myset}[2]{ \left\{ #1 \;\left|\; #2 \right. \right\} }
\newcommand{\mysetl}[2]{ \left\{\left. #1 \right| #2 \right\} }
\newcommand{\bval}[1]{[\![ #1 ]\!]}
\newcommand{\prefix}{\sqsubseteq}
\newcommand{\prprefix}{\underset{\neq}{\sqsubset}}
\newcommand{\st}{{\rm st}}
\newcommand{\diam}{\mathrm{diam}}
%\newcommand{\doublespace}{\renewcommand{\baselinestretch}{1.5}\normalsize}
\newcommand{\binary}{\{0,1\}^*}
\newcommand{\limn}{\lim\limits_{n\to\infty}}
\newcommand{\liminfn}{\liminf\limits_{n\to\infty}}
\newcommand{\limsupn}{\limsup\limits_{n\to\infty}}
\newcommand{\ith}{{i^{\mathrm{th}}}}
\renewcommand{\Pr}[2]{\underset{#1}{\mathrm{Prob}}\left[#2\right]}
\newcommand{\size}[1]{\parallel\negthinspace #1\negthinspace\parallel}
%\newcommand{\restr}{\mbox{\raisebox{.5mm}{$\upharpoonright$}}}
\newcommand{\restr}{\upharpoonright}
\newcommand{\vb}{{\vec{\beta}}}
\newcommand{\RANDb}{\RAND^\vb}

\newcommand{\join}{\oplus}
\newcommand{\TQBF}{{\rm TQBF}}
\newcommand{\GI}{{\rm GI}}
\newcommand{\parityP}{{\oplus\P}}
\newcommand{\sharpP}{{\#\P}}
\newcommand{\CeqP}{{{\rm C}_=\P}}
\newcommand{\MODkP}{{{\rm MOD}_k\P}}
\newcommand{\BP}{\mathrm{BP}\cdot}

% Blackboard Bold Sets
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}

% Measure and Dimension
\newcommand{\p}{{\mathrm{p}}}
\newcommand{\ptwo}{{\p_{\thinspace\negthinspace_2}}}
\newcommand{\pthree}{{\p_{\thinspace\negthinspace_3}}}
\newcommand{\pspace}{{\mathrm{pspace}}}
\newcommand{\ptwospace}{{\mathrm{p}_{\thinspace\negthinspace_2}\mathrm{space}}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\rec}{{\mathrm{rec}}}
\newcommand{\all}{{\mathrm{all}}}
\newcommand{\FS}{{\mathrm{FS}}}
\newcommand{\comp}{{\mathrm{comp}}}
\newcommand{\constr}{{\mathrm{constr}}}
\newcommand{\mup}{\mu_{\mathrm{p}}}
\newcommand{\dimall}{\dim_\all}
\newcommand{\dimp}{\dim_\p}
\newcommand{\dimfs}{\mathrm{dim}_\mathrm{FS}}
\newcommand{\dimpspace}{\mathrm{dim}_\mathrm{pspace}}
\newcommand{\dimh}{\mathrm{dim}_\mathrm{H}}
\newcommand{\dimrec}{\mathrm{dim}_\mathrm{rec}}
\newcommand{\dimcomp}{\mathrm{dim}_\comp}
\newcommand{\cdim}{\mathrm{cdim}}
\newcommand{\dimptwo}{\dim_\ptwo}
\newcommand{\dimpthree}{\dim_\pthree}
\newcommand{\dimptwospace}{\dim_\ptwospace}
\newcommand{\Dimptwo}{\Dim_\ptwo}
\newcommand{\Dimptwospace}{\Dim_\ptwospace}
\newcommand{\muptwo}{\mu_\ptwo}
\newcommand{\mupthree}{\mu_\pthree}
\newcommand{\Deltapthree}{{\Delta^\p_3}}
\newcommand{\dimDeltapthree}{\dim_\Deltapthree}
\newcommand{\Deltaptwo}{{\Delta^\p_2}}
\newcommand{\dimDeltaptwo}{\dim_\Deltaptwo}
\newcommand{\DeltaPtwo}{{\Delta^\P_2}}
\newcommand{\DeltaPthree}{{\Delta^\P_3}}

\renewcommand{\dim}{{\mathrm{dim}}}
\newcommand{\udim}{{\overline{\dim}}}
\newcommand{\ldim}{{\underline{\dim}}}
\newcommand{\dimpack}{{\dim}_{\mathrm{P}}}
\newcommand{\dimb}{{\dim}_{\mathrm{B}}}
\newcommand{\udimb}{{\udim}_{\mathrm{B}}}
\newcommand{\ldimb}{{\ldim}_{\mathrm{B}}}
\newcommand{\udimmb}{\udim_{\mathrm{MB}}}

\newcommand{\Dim}{{\mathrm{Dim}}}
\newcommand{\cDim}{{\mathrm{cDim}}}
\newcommand{\Dimfs}{{\Dim_\FS}}
\newcommand{\Dimp}{{\Dim_\p}}
\newcommand{\Dimcomp}{{\Dim_\comp}}
\newcommand{\Dimpspace}{{\Dim_\pspace}}

\newcommand{\str}{{\mathrm{str}}}
\newcommand{\regSS}{S^\infty}
\newcommand{\strSS}{S^\infty_{\mathrm{str}}}

\newcommand{\G}{{\mathcal{G}}}
\newcommand{\Ghat}{{\widehat{\G}}}
\newcommand{\hatG}{\Ghat}
\newcommand{\Gstr}{\G^{\mathrm{str}}}
\newcommand{\hatGstr}{\hatG^{\mathrm{str}}}

\newcommand{\D}{{\mathcal{D}}}
\newcommand{\Gconstr}{\mathcal{G}_\mathrm{constr}}
\newcommand{\hatGconstr}{\mathcal{\hatG}_\mathrm{constr}}
\newcommand{\Gstrconstr}{\mathcal{G}_\mathrm{constr}^\mathrm{str}}
\newcommand{\hatGstrconstr}{\mathcal{\hatG}_\mathrm{constr}^\mathrm{str}}

\newcommand{\C}{\mathbf{C}}
\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\FREQ}{{\mathrm{FREQ}}}
\newcommand{\freq}{{\mathrm{freq}}}

% Prediction
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\Pred}{\mathrm{Pred}}
\newcommand{\Predp}{\mathrm{Pred}_\p}
\newcommand{\predp}{\mathrm{pred}_\p}
\newcommand{\unpred}{\mathrm{unpred}}
\newcommand{\Unpred}{\mathrm{Unpred}}
\newcommand{\unpredlog}{\mathrm{unpred}^\mathrm{log}}
\newcommand{\Unpredlog}{\mathrm{Unpred}^\mathrm{log}}
\newcommand{\unpredlogp}{\mathrm{unpred}^\mathrm{log}_\mathrm{p}}
\newcommand{\unpredabs}{\mathrm{unpred}^\mathrm{abs}}
\newcommand{\unpredabsp}{\mathrm{unpred}^\mathrm{abs}_\mathrm{p}}
\newcommand{\predcomp}{\pred_\comp}
\newcommand{\predfs}{\pred_\mathrm{FS}}
\newcommand{\Ik}{{\cal I}_k}
\newcommand{\Ikbar}{\overline{\Ik}}
\newcommand{\Hk}{{\cal H}_k}

\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\logL}{\calL^{\log}}
\newcommand{\strlogL}{\calL^{\log}_{\str}}
\newcommand{\abs}{\mathrm{abs}}
\newcommand{\absL}{\calL^{\abs}}

\newcommand{\loss}{{\mathit{loss}}}
\newcommand{\losslog}{\loss^{\log}}
\newcommand{\lossabs}{\loss^\abs}


% Complexity Classes
\newcommand{\co}[1]{\mathrm{co}#1}
\newcommand{\strings}{\{0,1\}^*}
\newcommand{\ALL}{\mathrm{ALL}}
\newcommand{\RAND}{\mathrm{RAND}}
\newcommand{\RANDweak}{\mathrm{RAND}_\mathrm{weak}}
\newcommand{\DIM}{\mathrm{DIM}}
\newcommand{\DIMstr}{\DIM_\str}
\newcommand{\coDIM}{\mathrm{coDIM}}
\newcommand{\REC}{\mathrm{REC}}
\newcommand{\DEC}{\mathrm{DEC}}
\newcommand{\CE}{\mathrm{CE}}
\newcommand{\coCE}{\mathrm{coCE}}
\newcommand{\RE}{\mathrm{RE}}
\newcommand{\coRE}{\mathrm{coRE}}
\newcommand{\SPARSE}{\mathrm{SPARSE}}
\newcommand{\DENSE}{\mathrm{DENSE}}
\newcommand{\DENSEio}{\mathrm{DENSE}_\mathrm{i.o.}}
\newcommand{\DTIME}{\mathrm{DTIME}}
\newcommand{\NTIME}{\mathrm{NTIME}}
\newcommand{\DTIMEF}{\mathrm{DTIMEF}}
\newcommand{\NP}{{\ensuremath{\mathrm{NP}}}}
\newcommand{\coNP}{\co{\NP}}
\newcommand{\AM}{{\rm AM}}
\newcommand{\MA}{{\rm MA}}
\newcommand{\DeltaPTwo}{\Delta^{\mathrm{P}}_2}
\newcommand{\DP}{\mathrm{DP}}
\newcommand{\SUBEXP}{\mathrm{SUBEXP}}
\newcommand{\SIZE}{{\rm SIZE}}
\newcommand{\SIZEio}{\SIZE_{\rm i.o.}}
\newcommand{\NSIZE}{{\rm NSIZE}}
\newcommand{\NSIZEio}{\NSIZE_{\rm i.o.}}
\newcommand{\BPP}{{\rm BPP}}
\newcommand{\PF}{{\rm PF}}
\newcommand{\ZPP}{{\rm ZPP}}
\newcommand{\RP}{{\rm RP}}
\newcommand{\coRP}{\co{\RP}}
\newcommand{\APP}{{\rm APP}}
\newcommand{\AP}{{\rm AP}}
\newcommand{\E}{{\rm E}}
\newcommand{\NE}{{\rm NE}}
\newcommand{\EE}{{\rm EE}}
\newcommand{\ESPACE}{{\rm ESPACE}}
\newcommand{\PSPACE}{{\rm PSPACE}}
\renewcommand{\P}{\ensuremath{{\mathrm P}}}
\newcommand{\QP}{{\rm QP}}
\newcommand{\NQP}{{\rm NQP}}
\newcommand{\Etwo}{{\rm E_2}}
\newcommand{\Ethree}{{\rm E_3}}
\newcommand{\EtwoSPACE}{{\rm E_2SPACE}}
\newcommand{\EXP}{{\rm EXP}}
\newcommand{\NEXP}{{\rm NEXP}}
\newcommand{\DSPACE}{{\rm DSPACE}}
\newcommand{\DSPACEF}{{\rm DSPACEF}}
\newcommand{\NEE}{{\rm NEE}}
\newcommand{\Poly}{{\rm P}}
\newcommand{\Pc}{{\rm P}}
\newcommand{\PPoly}{{\rm {P/Poly}}}
\newcommand{\Psel}{{\rm {P-sel}}}
\newcommand{\WS}{{\rm WS}}
\newcommand{\Ei}{\E_i}
\newcommand{\EiSPACE}{\mathrm{E}_i\mathrm{SPACE}}
\newcommand{\EoneSPACE}{\mathrm{E}_1\mathrm{SPACE}}
\newcommand{\linear}{\mathrm{linear}}
\newcommand{\polynomial}{\mathrm{polynomial}}
\newcommand{\EXPSPACE}{\mathrm{EXPSPACE}}
\newcommand{\PP}{{\rm PP}}
\newcommand{\SPP}{{\rm SPP}}
\newcommand{\GapP}{{\rm GapP}}
\newcommand{\PH}{{\rm PH}}
\newcommand{\Ppoly}{{\rm P/poly}}
\newcommand{\EH}{{\rm EH}}
\newcommand{\EHsigmaone}{{\Sigma_1^\E}}
\newcommand{\EHsigmatwo}{{\Sigma_2^\E}}
\newcommand{\EHsigmathree}{{\Sigma_3^\E}}
\newcommand{\EHdeltaone}{{\Delta_1^\E}}
\newcommand{\EHdeltatwo}{{\Delta_2^\E}}
\newcommand{\EHdeltathree}{{\Delta_3^\E}}
\newcommand{\EHpione}{{\Pi_1^\E}}
\newcommand{\EHpitwo}{{\Pi_2^\E}}
\newcommand{\EHpithree}{{\Pi_3^\E}}
% Calligraphy
\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calP}{{\cal P}}

% Kolmogorov Complexity
\newcommand{\calKS}{{\cal KS}}
\newcommand{\calKT}{{\cal KT}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calCD}{{\cal CD}}
\newcommand{\calCND}{{\cal CND}}
\newcommand{\K}{{\mathrm{K}}}
\newcommand{\KS}{{\mathrm{KS}} }
\newcommand{\KT}{{\mathrm{KT}} }
\newcommand{\CD}{{\mathrm{CD}} }
\newcommand{\CND}{{\mathrm{CND}} }

% Reductions
\newcommand{\leqpm}{\leq^\p_\mathrm{m}}
\newcommand{\leqmp}{\leqpm}
\newcommand{\leqpT}{\leq^\mathrm{p}_\mathrm{T}}
\newcommand{\leqpr}{\leq^\mathrm{p}_r}
\newcommand{\leqonettp}{\leq_{1-\mathrm{tt}}^{\mathrm{P}}}
\newcommand{\murec}[1]{{\mu({#1}\mid \REC)}}
\newcommand{\muex}[1]{{\mu({#1}\mid \Etwo)}}
\newcommand{\redu}[2]{{\leq^{\rm {{#1}}}_{{\rm{#2}}}}}
\newcommand{\predu}[1]{{\redu{P}{#1}}}
\newcommand{\pmred}{{\predu{m}}}
\newcommand{\ptred}{{\predu{T}}}

%pair reductions

\newcommand{\leqppm}{\leq^{\p\p}_\mathrm{m}}
\newcommand{\leqppum}{\leq^{\p\p}_\mathrm{um}}

\newcommand{\leqppsm}{\leq^{\p\p}_\mathrm{sm}}
\newcommand{\leqppT}{\leq^{\mathrm{pp}}_\mathrm{T}}
\newcommand{\leqppuT}{\leq^{\mathrm{pp}}_\mathrm{uT}}



% Reduction Closures
\newcommand{\Pm}{\mathrm{P}_{\mathrm{m}}}
\newcommand{\PT}{\mathrm{P}_{\mathrm{T}}}
\newcommand{\Ptt}{\mathrm{P}_{\mathrm{tt}}}
\newcommand{\Pctt}{\mathrm{P}_{\mathrm{ctt}}}
\newcommand{\Pdtt}{\mathrm{P}_{\mathrm{dtt}}}
\newcommand{\Ponett}{\mathrm{P}_{1-\mathrm{tt}}}
\newcommand{\Pmi}{\Pm^{-1}}
\renewcommand{\Pr}{\mathrm{P}_r}
\newcommand{\Pri}{\Pr^{-1}}
% Degrees
\newcommand{\degpm}{\mathrm{deg}^{\mathrm{p}}_{\mathrm{m}}}
\newcommand{\degpr}{\mathrm{deg}^\mathrm{p}_r}
\newcommand{\equivpm}{\equiv^\p_\mathrm{m}}
% Hard and Complete sets
\newcommand{\m}{\mathrm{m}}
\newcommand{\Cpm}{\calC^\p_\m}
\newcommand{\Hpm}{\calH^\p_\m}
\newcommand{\Cpr}{\calC^\p_r}
\newcommand{\Hpr}{\calH^\p_r}

% Stuff from CPED
\newcommand{\CH}{\mathcal{H}}
\newcommand{\CHdec}{\mathcal{H}_\DEC}
\newcommand{\CHce}{\mathcal{H}_\CE}
\newcommand{\Pione}{\Pi^0_1}
\newcommand{\Pitwo}{\Pi^0_2}
\newcommand{\BorelPi}[2]{{\bf \Pi}^ #1 _#2}
\newcommand{\BorelSigma}[2]{{\bf \Sigma}^ #1_#2}
\newcommand{\Sigmaone}{\Sigma^0_1}
\newcommand{\Sigmatwo}{\Sigma^0_2}
\newcommand{\PioneC}{\Pione}% \upharpoonright \C}
\newcommand{\PitwoC}{\Pitwo}% \upharpoonright \C}
\newcommand{\SigmaoneC}{\Sigmaone}% \upharpoonright \C}
\newcommand{\SigmatwoC}{\Sigmatwo}% \upharpoonright \C}
\newcommand{\io}{{\mathrm{i.o.}}}
\newcommand{\aev}{{\mathrm{a.e.}}}
\newcommand{\ioA}{A^\io}
\newcommand{\ioB}{B^\io}
\newcommand{\ioC}{C^\io}
\newcommand{\aeA}{A^\aev}
\newcommand{\aeB}{B^\aev}


% Names
\newcommand{\MartinLof}{Martin-L\"{o}f}

\newcommand{\nth}{n^{\mathrm{th}}}


\newcommand{\supp}{\mathrm{supp}}
\newcommand{\eH}{\mathrm{H}}


%Dimension Entropy Rate
\newcommand{\SpanP}{\mathrm{SpanP}}


\newcommand{\length}[1]{\lvert #1 \rvert}


==> numbering.tex <==
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{claim}{Claim}

\newenvironment{theorem_cite}[1]
{\begin{theorem}  {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_cite}[1]
{\begin{lemma}  {\rm (#1)}}
{\end{lemma}}
\newenvironment{corollary_cite}[1]
{\begin{corollary}  {\rm (#1)}}
{\end{corollary}}
\newenvironment{proposition_cite}[1]
{\begin{proposition}  {\rm (#1)}}
{\end{proposition}}

\newenvironment{theorem_named}[1]
{\begin{theorem} {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_named}[1]
{\begin{lemma} {\rm (#1)}}
{\end{lemma}}

\newenvironment{proof_claim}
{\noindent{\em Proof of Claim.}}
{\hfill $\square$ {\em Claim.}}

\newenvironment{Proof}
{\begin{proof}}
{\end{proof}}

\newenvironment{Proofnamed}[1]
{\begin{proof}[Proof #1.]}
{\end{proof}}

\newenvironment{pf}
{\begin{proof}[Pf.]}
{\end{proof}}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{observations}[theorem]{Observations}

\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{question}[theorem]{Question}

\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}

\newtheorem{problem}[theorem]{Problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem*{definition}{Definition}
\newtheorem*{defn}{Definition}
\newtheorem*{definitions}{Definitions}

\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem*{example*}{Example}
\newtheorem*{examples*}{Examples}

\newenvironment{example_cite}[1]
{\begin{example}  {\rm (#1)}}
{\end{example}}

\newtheorem{construction}[theorem]{Construction}
\newtheorem{extension}[theorem]{Extension}

\newtheorem*{remarks}{Remarks}
\newtheorem*{remark}{Remark}

\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}

\newtheorem*{ack}{Acknowledgment}
\newtheorem*{acks}{Acknowledgments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}
\numberwithin{figure}{section}


==> renumbering.tex <==
\usepackage{amsthm}

\renewtheorem{theorem}{Theorem}[section]
\renewtheorem{corollary}[theorem]{Corollary}
\renewtheorem{lemma}[theorem]{Lemma}
\renewtheorem{proposition}[theorem]{Proposition}
\newtheorem*{claim}{Claim}

\newenvironment{theorem_cite}[1]
{\begin{theorem}  {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_cite}[1]
{\begin{lemma}  {\rm (#1)}}
{\end{lemma}}
\newenvironment{corollary_cite}[1]
{\begin{corollary}  {\rm (#1)}}
{\end{corollary}}
\newenvironment{proposition_cite}[1]
{\begin{proposition}  {\rm (#1)}}
{\end{proposition}}

\newenvironment{theorem_named}[1]
{\begin{theorem} {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_named}[1]
{\begin{lemma} {\rm (#1)}}
{\end{lemma}}

\newenvironment{proof_claim}
{\noindent{\em Proof of Claim.}}
{\hfill $\square$ {\em Claim.}}

\newenvironment{Proof}
{\begin{proof}}
{\end{proof}}

\newenvironment{Proofnamed}[1]
{\begin{proof}[Proof #1.]}
{\end{proof}}

\newenvironment{pf}
{\begin{proof}[Pf.]}
{\end{proof}}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{observations}[theorem]{Observations}

\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{question}[theorem]{Question}

\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}

\newtheorem{problem}[theorem]{Problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem*{definition}{Definition}
\newtheorem*{defn}{Definition}
\newtheorem*{definitions}{Definitions}

\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem*{example*}{Example}
\newtheorem*{examples*}{Examples}

\newenvironment{example_cite}[1]
{\begin{example}  {\rm (#1)}}
{\end{example}}

\newtheorem{construction}[theorem]{Construction}
\newtheorem{extension}[theorem]{Extension}

\newtheorem*{remarks}{Remarks}
\newtheorem*{remark}{Remark}

\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}

\newtheorem*{ack}{Acknowledgment}
\newtheorem*{acks}{Acknowledgments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}
\numberwithin{figure}{section}


==> section2.tex <==
\section{Preliminaries}\label{se:preliminaries}
Let $m\geq 2$ be an integer. We work with the $m$-ary alphabet $\Sigma_m=\{ 0,1, \dots, m-1\}$.
$\Sigma_m^*$ is the set of all (finite) {\em strings} on $\Sigma_m$ including the empty string $\lambda$.
$\C_m =\Sigma_m^\infty$ is the of all (infinite) $m$-ary {\em sequences}. $\C=\C_2$ is the Cantor space.
$\Delta(\Sigma_m)$ is the set of all probability measures on $\Sigma_m$.

Let $i$ be an integer such that $0\leq i\leq m-1$.
The symbol counting function $\#_i:(\C_m\cup \Sigma_m^*)\times \N\rightarrow \N$
is defined such that for every string or sequence $S$ and $n\in\N$,
$\#_i(S, n)$ is the number of occurrences of $i$ in the first $n$ bits of $S$.
The symbol frequency function $\pi_i:(\C_m\cup \Sigma_m^*)\times \N \rightarrow [0,1]$
is defined such that $\pi_i(S, n) = \#_i(S,n)/n$.
The empirical measure function $\vec\pi:(\C_m\cup\Sigma_m^*)\times \N\rightarrow\Delta(\Sigma_m)$
is defined such that $\vec\pi(S, n)= (\pi_0(S,n), \dots, \pi_{m-1}(S,n))$.
Intuitively, $\vec\pi$ extracts empirical probability measures from the first $n$ bits
of a string or a sequence based on the actual frequencies of digits. 

==> singlenumbering.tex <==
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{claim}{Claim}

\newenvironment{theorem_cite}[1]
{\begin{theorem}  {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_cite}[1]
{\begin{lemma}  {\rm (#1)}}
{\end{lemma}}
\newenvironment{corollary_cite}[1]
{\begin{corollary}  {\rm (#1)}}
{\end{corollary}}
\newenvironment{proposition_cite}[1]
{\begin{proposition}  {\rm (#1)}}
{\end{proposition}}

\newenvironment{theorem_named}[1]
{\begin{theorem} {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_named}[1]
{\begin{lemma} {\rm (#1)}}
{\end{lemma}}

\newenvironment{proof_claim}
{\noindent{\em Proof of Claim.}}
{\hfill $\square$ {\em Claim.}}

\newenvironment{Proof}
{\begin{proof}}
{\end{proof}}

\newenvironment{Proofnamed}[1]
{\begin{proof}[Proof #1.]}
{\end{proof}}

\newenvironment{pf}
{\begin{proof}[Pf.]}
{\end{proof}}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{observations}[theorem]{Observations}

\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{question}[theorem]{Question}

\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}

\newtheorem{problem}[theorem]{Problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem*{definition}{Definition}
\newtheorem*{defn}{Definition}
\newtheorem*{definitions}{Definitions}

\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem*{example*}{Example}
\newtheorem*{examples*}{Examples}

\newenvironment{example_cite}[1]
{\begin{example}  {\rm (#1)}}
{\end{example}}

\newtheorem{construction}[theorem]{Construction}
\newtheorem{extension}[theorem]{Extension}

\newtheorem*{remarks}{Remarks}
\newtheorem*{remark}{Remark}

\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}

\newtheorem*{ack}{Acknowledgment}
\newtheorem*{acks}{Acknowledgments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\numberwithin{equation}{section}
%\numberwithin{figure}{section}

